Real-time Discovery of AT2020xnd: A Fast, Luminous Ultraviolet Transient with Minimal Radioactive Ejecta

The many unusual properties of the enigmatic AT2018cow suggested that at least some subset of the empirical class of fast blue optical transients (FBOTs) represents a genuinely new astrophysical phenomenon. Unfortunately, the intrinsic rarity and fleeting nature of these events have made it difficult to identify additional examples early enough to acquire the observations necessary to constrain theoretical models. We present here the Zwicky Transient Facility discovery of AT2020xnd (ZTF20acigmel, the "Camel") at z=0.243, the first unambiguous AT2018cow analog to be found and confirmed in real time. AT2018cow and AT2020xnd share all key observational properties: a fast optical rise, sustained high photospheric temperature, absence of a second peak attributable to ejection of a radioactively-heated stellar envelope, extremely luminous radio, millimetre, and X-ray emission, and a dwarf-galaxy host. This supports the argument that AT2018cow-like events represent a distinct phenomenon from slower-evolving radio-quiet supernovae, likely requiring a different progenitor or a different central engine. The sample properties of the four known members of this class to date disfavour tidal disruption models but are consistent with the alternative model of an accretion powered jet following the direct collapse of a massive star to a black hole. Contextual filtering of alert streams combined with rapid photometric verification using multi-band imaging provides an efficient way to identify future members of this class, even at high redshift.

==> ref.tex <==
\begin{thebibliography}{}
\makeatletter
\relax
\def\mn@urlcharsother{\let\do\@makeother \do\$\do\&\do\#\do\^\do\_\do\%\do\~}
\def\mn@doi{\begingroup\mn@urlcharsother \@ifnextchar [ {\mn@doi@}
  {\mn@doi@[]}}
\def\mn@doi@[#1]#2{\def\@tempa{#1}\ifx\@tempa\@empty \href
  {http://dx.doi.org/#2} {doi:#2}\else \href {http://dx.doi.org/#2} {#1}\fi
  \endgroup}
\def\mn@eprint#1#2{\mn@eprint@#1:#2::\@nil}
\def\mn@eprint@arXiv#1{\href {http://arxiv.org/abs/#1} {{\tt arXiv:#1}}}
\def\mn@eprint@dblp#1{\href {http://dblp.uni-trier.de/rec/bibtex/#1.xml}
  {dblp:#1}}
\def\mn@eprint@#1:#2:#3:#4\@nil{\def\@tempa {#1}\def\@tempb {#2}\def\@tempc
  {#3}\ifx \@tempc \@empty \let \@tempc \@tempb \let \@tempb \@tempa \fi \ifx
  \@tempb \@empty \def\@tempb {arXiv}\fi \@ifundefined
  {mn@eprint@\@tempb}{\@tempb:\@tempc}{\expandafter \expandafter \csname
  mn@eprint@\@tempb\endcsname \expandafter{\@tempc}}}

\bibitem[\protect\citeauthoryear{{Andreoni} et~al.,}{{Andreoni}
  et~al.}{2020}]{Andreoni2020}
{Andreoni} I.,  et~al., 2020, \mn@doi [\apj] {10.3847/1538-4357/abbf4c}, \href
  {https://ui.adsabs.harvard.edu/abs/2020ApJ...904..155A} {904, 155}

\bibitem[\protect\citeauthoryear{{Arnett}}{{Arnett}}{1980}]{Arnett1980}
{Arnett} W.~D.,  1980, \mn@doi [\apj] {10.1086/157898}, \href
  {https://ui.adsabs.harvard.edu/abs/1980ApJ...237..541A} {237, 541}

\bibitem[\protect\citeauthoryear{{Arnett}}{{Arnett}}{1982}]{Arnett1982}
{Arnett} W.~D.,  1982, \mn@doi [\apj] {10.1086/159681}, \href
  {https://ui.adsabs.harvard.edu/abs/1982ApJ...253..785A} {253, 785}

\bibitem[\protect\citeauthoryear{{Bellm} et~al.,}{{Bellm}
  et~al.}{2019a}]{Bellm2019}
{Bellm} E.~C.,  et~al., 2019a, \mn@doi [\pasp] {10.1088/1538-3873/aaecbe},
  \href {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8002B} {131, 018002}

\bibitem[\protect\citeauthoryear{{Bellm} et~al.,}{{Bellm}
  et~al.}{2019b}]{Bellm2019surveys}
{Bellm} E.~C.,  et~al., 2019b, \mn@doi [\pasp] {10.1088/1538-3873/ab0c2a},
  \href {https://ui.adsabs.harvard.edu/abs/2019PASP..131f8003B} {131, 068003}

\bibitem[\protect\citeauthoryear{{Bietenholz} et~al.,}{{Bietenholz}
  et~al.}{2020}]{Bietenholz+2020}
{Bietenholz} M.~F.,  et~al., 2020, \mn@doi [\mnras] {10.1093/mnras/stz3249},
  \href {https://ui.adsabs.harvard.edu/abs/2020MNRAS.491.4735B} {491, 4735}

\bibitem[\protect\citeauthoryear{{Blagorodnova} et~al.,}{{Blagorodnova}
  et~al.}{2018}]{Blagorodnova+2018}
{Blagorodnova} N.,  et~al., 2018, \mn@doi [\pasp] {10.1088/1538-3873/aaa53f},
  \href {https://ui.adsabs.harvard.edu/abs/2018PASP..130c5003B} {130, 035003}

\bibitem[\protect\citeauthoryear{{Blanton}, {Kazin}, {Muna}, {Weaver}  \&
  {Price-Whelan}}{{Blanton} et~al.}{2011}]{Blanton+2011}
{Blanton} M.~R.,  {Kazin} E.,  {Muna} D.,  {Weaver} B.~A.,   {Price-Whelan} A.,
   2011, \mn@doi [\aj] {10.1088/0004-6256/142/1/31}, \href
  {https://ui.adsabs.harvard.edu/abs/2011AJ....142...31B} {142, 31}

\bibitem[\protect\citeauthoryear{{Coppejans} et~al.,}{{Coppejans}
  et~al.}{2020}]{Coppejans+2020}
{Coppejans} D.~L.,  et~al., 2020, \mn@doi [\apjl] {10.3847/2041-8213/ab8cc7},
  \href {https://ui.adsabs.harvard.edu/abs/2020ApJ...895L..23C} {895, L23}

\bibitem[\protect\citeauthoryear{{Dekany} et~al.,}{{Dekany}
  et~al.}{2020}]{Dekany2020}
{Dekany} R.,  et~al., 2020, \mn@doi [\pasp] {10.1088/1538-3873/ab4ca2}, \href
  {https://ui.adsabs.harvard.edu/abs/2020PASP..132c8001D} {132, 038001}

\bibitem[\protect\citeauthoryear{{Dessart}, {Hillier}, {Woosley}, {Livne},
  {Waldman}, {Yoon}  \& {Langer}}{{Dessart} et~al.}{2016}]{Dessart+2016}
{Dessart} L.,  {Hillier} D.~J.,  {Woosley} S.,  {Livne} E.,  {Waldman} R.,
  {Yoon} S.-C.,   {Langer} N.,  2016, \mn@doi [\mnras] {10.1093/mnras/stw418},
  \href {https://ui.adsabs.harvard.edu/abs/2016MNRAS.458.1618D} {458, 1618}

\bibitem[\protect\citeauthoryear{{Dey} et~al.,}{{Dey} et~al.}{2019}]{Dey+2019}
{Dey} A.,  et~al., 2019, \mn@doi [\aj] {10.3847/1538-3881/ab089d}, \href
  {https://ui.adsabs.harvard.edu/abs/2019AJ....157..168D} {157, 168}

\bibitem[\protect\citeauthoryear{{Drout} et~al.,}{{Drout}
  et~al.}{2014}]{Drout+2014}
{Drout} M.~R.,  et~al., 2014, \mn@doi [\apj] {10.1088/0004-637X/794/1/23},
  \href {https://ui.adsabs.harvard.edu/abs/2014ApJ...794...23D} {794, 23}

\bibitem[\protect\citeauthoryear{{Duev} et~al.,}{{Duev}
  et~al.}{2019}]{Duev2019}
{Duev} D.~A.,  et~al., 2019, \mn@doi [\mnras] {10.1093/mnras/stz2357}, \href
  {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489.3582D} {489, 3582}

\bibitem[\protect\citeauthoryear{{Flewelling} et~al.,}{{Flewelling}
  et~al.}{2020}]{Flewelling+2020}
{Flewelling} H.~A.,  et~al., 2020, \mn@doi [\apjs] {10.3847/1538-4365/abb82d},
  \href {https://ui.adsabs.harvard.edu/abs/2020ApJS..251....7F} {251, 7}

\bibitem[\protect\citeauthoryear{{Foley} et~al.,}{{Foley}
  et~al.}{2003}]{Foley2003}
{Foley} R.~J.,  et~al., 2003, \mn@doi [\pasp] {10.1086/378242}, \href
  {https://ui.adsabs.harvard.edu/abs/2003PASP..115.1220F} {115, 1220}

\bibitem[\protect\citeauthoryear{{Fox} \& {Smith}}{{Fox} \&
  {Smith}}{2019}]{Fox+2019}
{Fox} O.~D.,  {Smith} N.,  2019, \mn@doi [\mnras] {10.1093/mnras/stz1925},
  \href {https://ui.adsabs.harvard.edu/abs/2019MNRAS.488.3772F} {488, 3772}

\bibitem[\protect\citeauthoryear{{Fremling} et~al.,}{{Fremling}
  et~al.}{2016}]{Fremling+2016}
{Fremling} C.,  et~al., 2016, \mn@doi [\aap] {10.1051/0004-6361/201628275},
  \href {https://ui.adsabs.harvard.edu/abs/2016A&A...593A..68F} {593, A68}

\bibitem[\protect\citeauthoryear{{Fremling} et~al.,}{{Fremling}
  et~al.}{2019}]{Fremling2019}
{Fremling} C.,  et~al., 2019, \mn@doi [\apjl] {10.3847/2041-8213/ab218f}, \href
  {https://ui.adsabs.harvard.edu/abs/2019ApJ...878L...5F} {878, L5}

\bibitem[\protect\citeauthoryear{{Graham} et~al.,}{{Graham}
  et~al.}{2019}]{Graham2019}
{Graham} M.~J.,  et~al., 2019, \mn@doi [\pasp] {10.1088/1538-3873/ab006c},
  \href {https://ui.adsabs.harvard.edu/abs/2019PASP..131g8001G} {131, 078001}

\bibitem[\protect\citeauthoryear{{Hamuy}}{{Hamuy}}{2003}]{Hamuy2003}
{Hamuy} M.,  2003, \mn@doi [\apj] {10.1086/344689}, \href
  {https://ui.adsabs.harvard.edu/abs/2003ApJ...582..905H} {582, 905}

\bibitem[\protect\citeauthoryear{{Ho} et~al.,}{{Ho} et~al.}{2019}]{Ho+2019}
{Ho} A. Y.~Q.,  et~al., 2019, \mn@doi [\apj] {10.3847/1538-4357/aaf473}, \href
  {https://ui.adsabs.harvard.edu/abs/2019ApJ...871...73H} {871, 73}

\bibitem[\protect\citeauthoryear{{Ho}, {Perley}  \& {Yao}}{{Ho}
  et~al.}{2020a}]{TNS204}
{Ho} A.~Y.~Q.,  {Perley} D.~A.,   {Yao} Y.,  2020a, Transient Name Server
  AstroNote, \href {https://ui.adsabs.harvard.edu/abs/2020TNSAN.204....1H}
  {204, 1}

\bibitem[\protect\citeauthoryear{{Ho} et~al.,}{{Ho} et~al.}{2020b}]{Ho+2020}
{Ho} A. Y.~Q.,  et~al., 2020b, \mn@doi [\apj] {10.3847/1538-4357/ab8bcf}, \href
  {https://ui.adsabs.harvard.edu/abs/2020ApJ...895...49H} {895, 49}

\bibitem[\protect\citeauthoryear{{Ho} et~al.,}{{Ho} et~al.}{2021}]{Ho+2021}
{Ho} A. Y.~Q.,  et~al., 2021, arXiv e-prints, \href
  {https://ui.adsabs.harvard.edu/abs/2021arXiv210508811H} {p. arXiv:2105.08811}

\bibitem[\protect\citeauthoryear{{Huang} et~al.,}{{Huang}
  et~al.}{2019}]{Huang+2019}
{Huang} K.,  et~al., 2019, \mn@doi [\apjl] {10.3847/2041-8213/ab23fd}, \href
  {https://ui.adsabs.harvard.edu/abs/2019ApJ...878L..25H} {878, L25}

\bibitem[\protect\citeauthoryear{{Inserra}}{{Inserra}}{2019}]{Inserra2019}
{Inserra} C.,  2019, \mn@doi [Nature Astronomy] {10.1038/s41550-019-0854-4},
  \href {https://ui.adsabs.harvard.edu/abs/2019NatAs...3..697I} {3, 697}

\bibitem[\protect\citeauthoryear{{Kasliwal} et~al.,}{{Kasliwal}
  et~al.}{2019}]{Kasliwal2019}
{Kasliwal} M.~M.,  et~al., 2019, \mn@doi [\pasp] {10.1088/1538-3873/aafbc2},
  \href {https://ui.adsabs.harvard.edu/abs/2019PASP..131c8003K} {131, 038003}

\bibitem[\protect\citeauthoryear{{Khatami} \& {Kasen}}{{Khatami} \&
  {Kasen}}{2019}]{Khatami2019}
{Khatami} D.~K.,  {Kasen} D.~N.,  2019, \mn@doi [\apj]
  {10.3847/1538-4357/ab1f09}, \href
  {https://ui.adsabs.harvard.edu/abs/2019ApJ...878...56K} {878, 56}

\bibitem[\protect\citeauthoryear{{Kremer}, {Lu}, {Piro}, {Chatterjee}, {Rasio}
  \& {Ye}}{{Kremer} et~al.}{2021}]{Kremer+2021}
{Kremer} K.,  {Lu} W.,  {Piro} A.~L.,  {Chatterjee} S.,  {Rasio} F.~A.,   {Ye}
  C.~S.,  2021, \mn@doi [\apj] {10.3847/1538-4357/abeb14}, \href
  {https://ui.adsabs.harvard.edu/abs/2021ApJ...911..104K} {911, 104}

\bibitem[\protect\citeauthoryear{{Kuin} et~al.,}{{Kuin}
  et~al.}{2019}]{Kuin+2019}
{Kuin} N. P.~M.,  et~al., 2019, \mn@doi [\mnras] {10.1093/mnras/stz053}, \href
  {https://ui.adsabs.harvard.edu/abs/2019MNRAS.487.2505K} {487, 2505}

\bibitem[\protect\citeauthoryear{{Lee} et~al.,}{{Lee} et~al.}{2011}]{Lee+2011}
{Lee} J.~C.,  et~al., 2011, \mn@doi [\apjs] {10.1088/0067-0049/192/1/6}, \href
  {https://ui.adsabs.harvard.edu/abs/2011ApJS..192....6L} {192, 6}

\bibitem[\protect\citeauthoryear{{Leung}, {Blinnikov}, {Nomoto}, {Baklanov},
  {Sorokina}  \& {Tolstov}}{{Leung} et~al.}{2020}]{Leung+2020}
{Leung} S.-C.,  {Blinnikov} S.,  {Nomoto} K.,  {Baklanov} P.,  {Sorokina} E.,
  {Tolstov} A.,  2020, \mn@doi [\apj] {10.3847/1538-4357/abba33}, \href
  {https://ui.adsabs.harvard.edu/abs/2020ApJ...903...66L} {903, 66}

\bibitem[\protect\citeauthoryear{{Leung}, {Fuller}  \& {Nomoto}}{{Leung}
  et~al.}{2021}]{Leung+2021}
{Leung} S.-C.,  {Fuller} J.,   {Nomoto} K.,  2021, \mn@doi [\apj]
  {10.3847/1538-4357/abfcbe}, \href
  {https://ui.adsabs.harvard.edu/abs/2021ApJ...915...80L} {915, 80}

\bibitem[\protect\citeauthoryear{{Liu}, {Zhang}, {Wang}  \& {Dai}}{{Liu}
  et~al.}{2018}]{Liu+2018}
{Liu} L.-D.,  {Zhang} B.,  {Wang} L.-J.,   {Dai} Z.-G.,  2018, \mn@doi [\apjl]
  {10.3847/2041-8213/aaeff6}, \href
  {https://ui.adsabs.harvard.edu/abs/2018ApJ...868L..24L} {868, L24}

\bibitem[\protect\citeauthoryear{{Lyman}, {Galbany}, {S{\'a}nchez}, {Anderson},
  {Kuncarayakti}  \& {Prieto}}{{Lyman} et~al.}{2020}]{Lyman+2020}
{Lyman} J.~D.,  {Galbany} L.,  {S{\'a}nchez} S.~F.,  {Anderson} J.~P.,
  {Kuncarayakti} H.,   {Prieto} J.~L.,  2020, \mn@doi [\mnras]
  {10.1093/mnras/staa1243}, \href
  {https://ui.adsabs.harvard.edu/abs/2020MNRAS.495..992L} {495, 992}

\bibitem[\protect\citeauthoryear{{Lyutikov} \& {Toonen}}{{Lyutikov} \&
  {Toonen}}{2019}]{Lyutikov+2019}
{Lyutikov} M.,  {Toonen} S.,  2019, \mn@doi [\mnras] {10.1093/mnras/stz1640},
  \href {https://ui.adsabs.harvard.edu/abs/2019MNRAS.487.5618L} {487, 5618}

\bibitem[\protect\citeauthoryear{{Mahabal} et~al.,}{{Mahabal}
  et~al.}{2019}]{Mahabal2019}
{Mahabal} A.,  et~al., 2019, \mn@doi [\pasp] {10.1088/1538-3873/aaf3fa}, \href
  {https://ui.adsabs.harvard.edu/abs/2019PASP..131c8002M} {131, 038002}

\bibitem[\protect\citeauthoryear{{Margutti} et~al.,}{{Margutti}
  et~al.}{2019}]{Margutti+2019}
{Margutti} R.,  et~al., 2019, \mn@doi [\apj] {10.3847/1538-4357/aafa01}, \href
  {https://ui.adsabs.harvard.edu/abs/2019ApJ...872...18M} {872, 18}

\bibitem[\protect\citeauthoryear{{Masci} et~al.,}{{Masci}
  et~al.}{2019}]{Masci2019}
{Masci} F.~J.,  et~al., 2019, \mn@doi [\pasp] {10.1088/1538-3873/aae8ac}, \href
  {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8003M} {131, 018003}

\bibitem[\protect\citeauthoryear{{Matthews} et~al.,}{{Matthews}
  et~al.}{2020}]{TNS218}
{Matthews} D.,  et~al., 2020, Transient Name Server AstroNote, \href
  {https://ui.adsabs.harvard.edu/abs/2020TNSAN.218....1M} {218, 1}

\bibitem[\protect\citeauthoryear{{Mazzali} et~al.,}{{Mazzali}
  et~al.}{2002}]{Mazzali2002}
{Mazzali} P.~A.,  et~al., 2002, \mn@doi [\apjl] {10.1086/341504}, \href
  {https://ui.adsabs.harvard.edu/abs/2002ApJ...572L..61M} {572, L61}

\bibitem[\protect\citeauthoryear{{Mohan}, {An}  \& {Yang}}{{Mohan}
  et~al.}{2020}]{Mohan+2020}
{Mohan} P.,  {An} T.,   {Yang} J.,  2020, \mn@doi [\apjl]
  {10.3847/2041-8213/ab64d1}, \href
  {https://ui.adsabs.harvard.edu/abs/2020ApJ...888L..24M} {888, L24}

\bibitem[\protect\citeauthoryear{{Morokuma-Matsui} et~al.,}{{Morokuma-Matsui}
  et~al.}{2019}]{Morokuma+2019}
{Morokuma-Matsui} K.,  et~al., 2019, \mn@doi [\apjl]
  {10.3847/2041-8213/ab2915}, \href
  {https://ui.adsabs.harvard.edu/abs/2019ApJ...879L..13M} {879, L13}

\bibitem[\protect\citeauthoryear{{Oke} et~al.,}{{Oke} et~al.}{1995}]{Oke+1995}
{Oke} J.~B.,  et~al., 1995, \mn@doi [\pasp] {10.1086/133562}, \href
  {https://ui.adsabs.harvard.edu/abs/1995PASP..107..375O} {107, 375}

\bibitem[\protect\citeauthoryear{{Pastorello} et~al.,}{{Pastorello}
  et~al.}{2004}]{Pastorello+2004}
{Pastorello} A.,  et~al., 2004, \mn@doi [\mnras]
  {10.1111/j.1365-2966.2004.07173.x}, \href
  {https://ui.adsabs.harvard.edu/abs/2004MNRAS.347...74P} {347, 74}

\bibitem[\protect\citeauthoryear{{Pastorello} et~al.,}{{Pastorello}
  et~al.}{2007}]{Pastorello+2007}
{Pastorello} A.,  et~al., 2007, \mn@doi [\nat] {10.1038/nature05825}, \href
  {https://ui.adsabs.harvard.edu/abs/2007Natur.447..829P} {447, 829}

\bibitem[\protect\citeauthoryear{{Patterson} et~al.,}{{Patterson}
  et~al.}{2019}]{Patterson2019}
{Patterson} M.~T.,  et~al., 2019, \mn@doi [\pasp] {10.1088/1538-3873/aae904},
  \href {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8001P} {131, 018001}

\bibitem[\protect\citeauthoryear{{Perley}}{{Perley}}{2019}]{Perley2019}
{Perley} D.~A.,  2019, \mn@doi [\pasp] {10.1088/1538-3873/ab215d}, \href
  {https://ui.adsabs.harvard.edu/abs/2019PASP..131h4503P} {131, 084503}

\bibitem[\protect\citeauthoryear{{Perley} et~al.,}{{Perley}
  et~al.}{2019}]{Perley+2019}
{Perley} D.~A.,  et~al., 2019, \mn@doi [\mnras] {10.1093/mnras/sty3420}, \href
  {https://ui.adsabs.harvard.edu/abs/2019MNRAS.484.1031P} {484, 1031}

\bibitem[\protect\citeauthoryear{{Perley} et~al.,}{{Perley}
  et~al.}{2020}]{Perley+2020}
{Perley} D.~A.,  et~al., 2020, \mn@doi [\apj] {10.3847/1538-4357/abbd98}, \href
  {https://ui.adsabs.harvard.edu/abs/2020ApJ...904...35P} {904, 35}

\bibitem[\protect\citeauthoryear{{Piro} \& {Lu}}{{Piro} \&
  {Lu}}{2020}]{Piro+2020}
{Piro} A.~L.,  {Lu} W.,  2020, \mn@doi [\apj] {10.3847/1538-4357/ab83f6}, \href
  {https://ui.adsabs.harvard.edu/abs/2020ApJ...894....2P} {894, 2}

\bibitem[\protect\citeauthoryear{{Prentice} et~al.,}{{Prentice}
  et~al.}{2018}]{Prentice+2018}
{Prentice} S.~J.,  et~al., 2018, \mn@doi [\apjl] {10.3847/2041-8213/aadd90},
  \href {https://ui.adsabs.harvard.edu/abs/2018ApJ...865L...3P} {865, L3}

\bibitem[\protect\citeauthoryear{{Pursiainen} et~al.,}{{Pursiainen}
  et~al.}{2018}]{Pursiainen+2018}
{Pursiainen} M.,  et~al., 2018, \mn@doi [\mnras] {10.1093/mnras/sty2309}, \href
  {https://ui.adsabs.harvard.edu/abs/2018MNRAS.481..894P} {481, 894}

\bibitem[\protect\citeauthoryear{{Quataert}, {Lecoanet}  \&
  {Coughlin}}{{Quataert} et~al.}{2019}]{Quataert+2019}
{Quataert} E.,  {Lecoanet} D.,   {Coughlin} E.~R.,  2019, \mn@doi [\mnras]
  {10.1093/mnrasl/slz031}, \href
  {https://ui.adsabs.harvard.edu/abs/2019MNRAS.485L..83Q} {485, L83}

\bibitem[\protect\citeauthoryear{{Rest} et~al.,}{{Rest}
  et~al.}{2018}]{Rest+2018}
{Rest} A.,  et~al., 2018, \mn@doi [Nature Astronomy]
  {10.1038/s41550-018-0423-2}, \href
  {https://ui.adsabs.harvard.edu/abs/2018NatAs...2..307R} {2, 307}

\bibitem[\protect\citeauthoryear{{Rivera Sandoval}, {Maccarone}, {Corsi},
  {Brown}, {Pooley}  \& {Wheeler}}{{Rivera Sandoval}
  et~al.}{2018}]{Rivera+2018}
{Rivera Sandoval} L.~E.,  {Maccarone} T.~J.,  {Corsi} A.,  {Brown} P.~J.,
  {Pooley} D.,   {Wheeler} J.~C.,  2018, \mn@doi [\mnras]
  {10.1093/mnrasl/sly145}, \href
  {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480L.146R} {480, L146}

\bibitem[\protect\citeauthoryear{{Schlafly} \& {Finkbeiner}}{{Schlafly} \&
  {Finkbeiner}}{2011}]{Schlafly+2011}
{Schlafly} E.~F.,  {Finkbeiner} D.~P.,  2011, \mn@doi [\apj]
  {10.1088/0004-637X/737/2/103}, \href
  {https://ui.adsabs.harvard.edu/abs/2011ApJ...737..103S} {737, 103}

\bibitem[\protect\citeauthoryear{{Smartt} et~al.,}{{Smartt}
  et~al.}{2015}]{Smartt+2015}
{Smartt} S.~J.,  et~al., 2015, \mn@doi [\aap] {10.1051/0004-6361/201425237},
  \href {https://ui.adsabs.harvard.edu/abs/2015A&A...579A..40S} {579, A40}

\bibitem[\protect\citeauthoryear{{Soker}, {Grichener}  \& {Gilkis}}{{Soker}
  et~al.}{2019}]{Soker+2019}
{Soker} N.,  {Grichener} A.,   {Gilkis} A.,  2019, \mn@doi [\mnras]
  {10.1093/mnras/stz364}, \href
  {https://ui.adsabs.harvard.edu/abs/2019MNRAS.484.4972S} {484, 4972}

\bibitem[\protect\citeauthoryear{{Steele} et~al.,}{{Steele}
  et~al.}{2004}]{Steele2004}
{Steele} I.~A.,  et~al., 2004, in {Oschmann} Jr. J.~M.,  ed.,  \procspie Vol.
  5489, Ground-based Telescopes. pp 679--692, \mn@doi{10.1117/12.551456}

\bibitem[\protect\citeauthoryear{{Tachibana} \& {Miller}}{{Tachibana} \&
  {Miller}}{2018}]{Tachibana2018}
{Tachibana} Y.,  {Miller} A.~A.,  2018, \mn@doi [\pasp]
  {10.1088/1538-3873/aae3d9}, \href
  {https://ui.adsabs.harvard.edu/abs/2018PASP..130l8001T} {130, 128001}

\bibitem[\protect\citeauthoryear{{Taggart} \& {Perley}}{{Taggart} \&
  {Perley}}{2021}]{Taggart+2021}
{Taggart} K.,  {Perley} D.~A.,  2021, \mn@doi [\mnras] {10.1093/mnras/stab174},
  \href {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.3931T} {503, 3931}

\bibitem[\protect\citeauthoryear{{Uno} \& {Maeda}}{{Uno} \&
  {Maeda}}{2020a}]{Uno+2020a}
{Uno} K.,  {Maeda} K.,  2020a, \mn@doi [\apj] {10.3847/1538-4357/ab9632}, \href
  {https://ui.adsabs.harvard.edu/abs/2020ApJ...897..156U} {897, 156}

\bibitem[\protect\citeauthoryear{{Uno} \& {Maeda}}{{Uno} \&
  {Maeda}}{2020b}]{Uno+2020b}
{Uno} K.,  {Maeda} K.,  2020b, \mn@doi [\apjl] {10.3847/2041-8213/abca32},
  \href {https://ui.adsabs.harvard.edu/abs/2020ApJ...905L...5U} {905, L5}

\bibitem[\protect\citeauthoryear{{Villar}, {Berger}, {Metzger}  \&
  {Guillochon}}{{Villar} et~al.}{2017}]{Villar+2017}
{Villar} V.~A.,  {Berger} E.,  {Metzger} B.~D.,   {Guillochon} J.,  2017,
  \mn@doi [\apj] {10.3847/1538-4357/aa8fcb}, \href
  {https://ui.adsabs.harvard.edu/abs/2017ApJ...849...70V} {849, 70}

\bibitem[\protect\citeauthoryear{{Weiler}}{{Weiler}}{2003}]{Weiler2003}
{Weiler} K.,  2003, {Supernovae and Gamma-Ray Bursters}.
~ Vol. 598, Springer, \mn@doi{10.1007/3-540-45863-8}

\bibitem[\protect\citeauthoryear{{Weiler}, {Panagia}, {Montes}  \&
  {Sramek}}{{Weiler} et~al.}{2002}]{Weiler2002}
{Weiler} K.~W.,  {Panagia} N.,  {Montes} M.~J.,   {Sramek} R.~A.,  2002,
  \mn@doi [\araa] {10.1146/annurev.astro.40.060401.093744}, \href
  {https://ui.adsabs.harvard.edu/abs/2002ARA&A..40..387W} {40, 387}

\bibitem[\protect\citeauthoryear{{Wiseman} et~al.,}{{Wiseman}
  et~al.}{2020}]{Wiseman+2020}
{Wiseman} P.,  et~al., 2020, \mn@doi [\mnras] {10.1093/mnras/staa2474}, \href
  {https://ui.adsabs.harvard.edu/abs/2020MNRAS.498.2575W} {498, 2575}

\bibitem[\protect\citeauthoryear{{Xiang} et~al.,}{{Xiang}
  et~al.}{2021}]{Xiang2021}
{Xiang} D.,  et~al., 2021, \mn@doi [\apj] {10.3847/1538-4357/abdeba}, \href
  {https://ui.adsabs.harvard.edu/abs/2021ApJ...910...42X} {910, 42}

\bibitem[\protect\citeauthoryear{Zampieri}{Zampieri}{2017}]{Zampieri2017}
Zampieri L.,  2017, in Alsabti A.~W.,  Murdin P.,  eds, , Handbook of
  Supernovae.
Springer International Publishing, Cham, pp 1--32,
  \mn@doi{10.1007/978-3-319-20794-0_26-1}, \url
  {https://doi.org/10.1007/978-3-319-20794-0_26-1}

\bibitem[\protect\citeauthoryear{{Zhou} et~al.,}{{Zhou}
  et~al.}{2021}]{Zhou+2021}
{Zhou} R.,  et~al., 2021, \mn@doi [\mnras] {10.1093/mnras/staa3764}, \href
  {https://ui.adsabs.harvard.edu/abs/2021MNRAS.501.3309Z} {501, 3309}

\makeatother
\end{thebibliography}

